Tetris is Hard, Even to Approximate

In the popular computer game of Tetris, the player is given a sequence of tetromino pieces and must pack them into a rectangular gameboard initially occupied by a given configuration of filled squares; any completely filled row of the gameboard is cleared and all pieces above it drop by one row. We prove that in the offline version of Tetris, it is NP-complete to maximize the number of cleared rows, maximize the number of tetrises (quadruples of rows simultaneously filled and cleared), minimize the maximum height of an occupied square, or maximize the number of pieces placed before the game ends. We furthermore show the extreme inapproximability of the first and last of these objectives to within a factor of p^(1-epsilon), when given a sequence of p pieces, and the inapproximability of the third objective to within a factor of (2 - epsilon), for any epsilon>0. Our results hold under several variations on the rules of Tetris, including different models of rotation, limitations on player agility, and restricted piece sets.

==> figures/configs/dead1.tex <==
\ifredraw
\psset{unit=0.06in}
\begin{tabular}{lllllllllllll}
  \begin{block}{7}{8}
    \column{5}{8}
    \piece{\floor[lightgray]044}00
  \end{block}
  &
  \begin{block}{7}{8}
    \column{5}{8}
    \piece{\floor[lightgray]440}00
  \end{block}
  &
  \begin{block}{7}{8}
    \column{5}{8}
    \piece{\floor[lightgray]666}00
    \piece{\LGr[lightgray]}24
  \end{block}
  &
  \begin{block}{7}{14}
    \column{5}{14}
    \piece{\floor[lightgray]099}00
    \piece{\LGr[lightgray]}24
  \end{block}
\\\\
\begin{block}{5}{8}
  \column{5}{8}
  \piece{\floor[lightgray]444}00
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]840}00
  \end{block}
&
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[green]}2{10}
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]840}00
    \piece{\LGr[green]}2{10}
  \end{block}
  &
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}2{22}
  \end{block}
&
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}2{22}
  \end{block}
  \\\\
  (a) & (b) & (c) & (d) & (e) & (f) & (g) 
\\\\
\end{tabular}

\else
\includegraphics{figures/configs/dead1.epsi.clean}
\fi

%\newcommand{\ipreppedlg}[1]{($\tI$-UP-$\tLG$-$#1$)\xspace}
%\newcommand{\lgpreppedlg}[2]{($\tLG$-UP-$\{#1,#2\}$)\xspace}
%\newcommand{\lgunderflat}[1]{($\tLG$-UF-$#1$)\xspace}
%\newcommand{\lgunapproachable}[1]{($\tLG$-UA-$#1$)\xspace}
%\newcommand{\lglgunapproachable}[2]{($\tLG$-UA-$\{#1,#2\}$)\xspace}
%\newcommand{\lgoverflatA}{($\tLG$-OF-1)\xspace}
%\newcommand{\lgoverflatB}{($\tLG$-OF-2)\xspace}
%\newcommand{\lgoverflatC}{($\tLG$-OF-3)\xspace}
%\newcommand{\lgoverflatD}[1]{($\tLG$-OF-4-$#1$)\xspace}
%\newcommand{\lgthappy}[1]{($\tLG$-TH-$#1$)\xspace}
%\newcommand{\lglgthappy}[2]{($\tLG$-TH-$\{#1,#2\}$)\xspace}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 


==> figures/configs/dead2.tex <==
\ifredraw
\begin{tabular}{lllllllllllll}
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]444}00
    \piece{\LGr[green]}2{10}
  \end{block}
&
\begin{block}{5}{14}
  \column{6}{14}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{17}
\end{block}
&
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]666}00
        \piece{\LGr[lightgray]}24
        \piece{\LGu[green]}06
      \end{block}
      &
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]666}00
        \piece{\LGr[lightgray]}24
        \piece{\LGu[green]}16
      \end{block}
&
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]666}00
        \piece{\LGr[lightgray]}24
        \piece{\LGr[green]}06
      \end{block}
      &
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]666}00
        \piece{\LGr[lightgray]}24
        \piece{\LGr[green]}2{10}
      \end{block}
  \\\\
  (h) & (i) & (j) & (k) & (l) & (m) & (n)
\\\\
\end{tabular}

\else
\includegraphics{figures/configs/dead2.epsi.clean}
\fi

%\newcommand{\ipreppedlg}[1]{($\tI$-UP-$\tLG$-$#1$)\xspace}
%\newcommand{\lgpreppedlg}[2]{($\tLG$-UP-$\{#1,#2\}$)\xspace}
%\newcommand{\lgunderflat}[1]{($\tLG$-UF-$#1$)\xspace}
%\newcommand{\lgunapproachable}[1]{($\tLG$-UA-$#1$)\xspace}
%\newcommand{\lglgunapproachable}[2]{($\tLG$-UA-$\{#1,#2\}$)\xspace}
%\newcommand{\lgoverflatA}{($\tLG$-OF-1)\xspace}
%\newcommand{\lgoverflatB}{($\tLG$-OF-2)\xspace}
%\newcommand{\lgoverflatC}{($\tLG$-OF-3)\xspace}
%\newcommand{\lgoverflatD}[1]{($\tLG$-OF-4-$#1$)\xspace}
%\newcommand{\lgthappy}[1]{($\tLG$-TH-$#1$)\xspace}
%\newcommand{\lglgthappy}[2]{($\tLG$-TH-$\{#1,#2\}$)\xspace}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 


==> figures/configs/dead3.tex <==
\ifredraw
\begin{tabular}{lllllllllllll}
  \begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]998}00
    \piece{\LGr[lightgray]}24
    \piece{\LGr[green]}2{16}
  \end{block}
&
      \begin{block}{5}{20}
        \column{5}{20}
        \piece{\floor[lightgray]998}00
        \piece{\LGr[lightgray]}24
        \piece{\LGr[green]}2{16}
        \piece{\LGr[green]}2{10}
      \end{block}
  &  
  \\\\
  (o) & (p) 
\\\\
\end{tabular}

\else
\includegraphics{figures/configs/dead3.epsi.clean}
\fi

%\newcommand{\ipreppedlg}[1]{($\tI$-UP-$\tLG$-$#1$)\xspace}
%\newcommand{\lgpreppedlg}[2]{($\tLG$-UP-$\{#1,#2\}$)\xspace}
%\newcommand{\lgunderflat}[1]{($\tLG$-UF-$#1$)\xspace}
%\newcommand{\lgunapproachable}[1]{($\tLG$-UA-$#1$)\xspace}
%\newcommand{\lglgunapproachable}[2]{($\tLG$-UA-$\{#1,#2\}$)\xspace}
%\newcommand{\lgoverflatA}{($\tLG$-OF-1)\xspace}
%\newcommand{\lgoverflatB}{($\tLG$-OF-2)\xspace}
%\newcommand{\lgoverflatC}{($\tLG$-OF-3)\xspace}
%\newcommand{\lgoverflatD}[1]{($\tLG$-OF-4-$#1$)\xspace}
%\newcommand{\lgthappy}[1]{($\tLG$-TH-$#1$)\xspace}
%\newcommand{\lglgthappy}[2]{($\tLG$-TH-$\{#1,#2\}$)\xspace}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 


==> figures/configs/unapproachable.tex <==
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
\end{block}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/notched/lg.tex <==
\ifredrawLGnotched
\begin{tabular}{llllllllllllll}
\iffalse
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGu[red]}04
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGu[red]}14
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGu[yellow]}1{12}
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[red]}02
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[red]}14
  \end{block}
  &
  \begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[green]}1{10}
  \end{block}
  &
  \begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[red]}2{14}
  \end{block}\\\\
  (h) & (h) & ($i$-v) & (h) & (h) & (1) & (h) \\\\
\fi
  \begin{block}{5}{10}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGl[red]}04
  \end{block}
  &
  \begin{block}{5}{10}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGl[red]}0{12}
  \end{block}
  &
  \begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[red]}04
  \end{block}
  &
  \begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[red]}14
  \end{block}
  &
  \begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[red]}0{12}
  \end{block}
  &
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[red]}1{22}
  \end{block}
  &
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}2{22}
  \end{block}
  \\\\
  (h)&(h)&(h)&(h)&(h)&(h)&(3)
\end{tabular}
\else
\includegraphics{figures/notched/lg.epsi.clean}
\includegraphics{figures/notched/lg.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rotations/lgtetris.tex <==
    \begin{tabular}[t]{cccccccccc}
~~~~$\longleftarrow$~~~~~
&
      \begin{block}33
        \piece{\annotation{\pspolygon(0,0)(3,0)(3,3)(0,3)}}00
        \piece{\LGd}00
      \end{block}
&
~~~~$\longleftrightarrow$~~~~
&
      \begin{block}33
        \piece{\annotation{\pspolygon(0,0)(3,0)(3,3)(0,3)}}00
        \piece{\LGl}01
      \end{block}
&
~~~~$\longleftrightarrow$~~~~
&
      \begin{block}33
        \piece{\annotation{\pspolygon(0,0)(3,0)(3,3)(0,3)}}00
        \piece{\LGu}00
      \end{block}
&
~~~~$\longleftrightarrow$~~~~
&
      \begin{block}33
        \piece{\annotation{\pspolygon(0,0)(3,0)(3,3)(0,3)}}00
        \piece{\LGr}01
      \end{block}
&
~~~~$\longrightarrow$~~~~
\\\\
    \end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> figures/rplat/rplat.tex <==
\ifredraw
\begin{tabular}{llll}
\begin{block}{5}{20}
  \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[lightgray]}2{10}
    \piece{\LGd[lightgray]}1{10}
    \piece{\Sq[red]}0{13}
  \end{block}
&
\begin{block}{5}{20}
  \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[lightgray]}2{10}
    \piece{\LGd[lightgray]}1{10}
    \piece{\Sq[green]}1{13}
  \end{block}
&
\begin{block}{5}{20}
  \column{5}{20}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[lightgray]}2{10}
    \piece{\LGd[lightgray]}1{10}
    \piece{\Sq[red]}0{13}
  \end{block}
&
\begin{block}{5}{20}
  \column{5}{20}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[lightgray]}2{10}
    \piece{\LGd[lightgray]}1{10}
    \piece{\Sq[green]}1{13}
  \end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/rplat/rplat.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/lgrtick.tex <==
\iftrue
\includegraphics{figures/rtick/lgrtick.epsi.clean}
\includegraphics{figures/rtick/lgrtick.epsi.clean}
\else
\newpage
\begin{tabular}{llllllllllllll}
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}02
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}14
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}24
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[yellow]}1{12}
% \end{block}
% &
% \begin{block}{5}{20}
%     \column{1}{20}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}2{16}
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}04
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}14
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}1{14}
% \end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGl[red]}04
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGl[red]}0{14}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGr[red]}04
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[red]}0{14}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[red]}1{18}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[green]}2{18}
\end{block}
\\\\
\end{tabular}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/lgrtick1.tex <==
\ifredraw
\begin{tabular}{llllllllllllll}
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGd[red]}02
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGd[red]}14
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGd[red]}2{10}
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGu[red]}04
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGu[red]}14
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGl[red]}04
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
  \piece{\LGr[red]}04
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[red]}1{12}
\end{block}
&
\begin{block}{5}{16}
    \column{1}{16}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[green]}2{12}
\end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/rtick/lgrtick1.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/lgrtick2.tex <==
\iftrue
\includegraphics{figures/rtick/lgrtick2.epsi.clean}
\includegraphics{figures/rtick/lgrtick2.epsi.clean}
\else
\newpage
\begin{tabular}{llllllllllllll}
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}02
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}14
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}24
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[yellow]}1{12}
% \end{block}
% &
% \begin{block}{5}{20}
%     \column{1}{20}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGd[red]}2{16}
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}04
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}14
% \end{block}
% &
% \begin{block}{5}{16}
%     \column{1}{16}
%     \piece{\LGr[green]}2{0}
%     \piece{\Sq[green]}1{2}
%     \piece{\LGr[green]}2{12}
%   \piece{\LGu[red]}1{14}
% \end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGl[red]}04
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGl[red]}0{14}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
  \piece{\LGr[red]}04
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[red]}0{14}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[red]}1{18}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[green]}2{0}
    \piece{\Sq[green]}1{2}
    \piece{\LGr[green]}2{12}
    \piece{\LGr[green]}2{18}
\end{block}
\\\\
\end{tabular}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/lsrticknotch.tex <==
\ifredraw
\begin{tabular}{llllllllllllll}
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSd[red]}03
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSd[red]}14
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSd[yellow]}1{13}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSl[red]}04
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSl[red]}0{14}
\end{block}
&
\begin{block}{5}{20}
    \column{1}{20}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\LGr[lightgray]}2{12}
    \piece{\LSl[red]}1{18}
\end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/rtick/lsrticknotch.epsi.clean}
\fi

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/rtickbot.tex <==
\begin{tabular}{llll}
\begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}24
    \piece{\Sq[red]}04
  \end{block}
&
\begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}24
    \piece{\Sq[yellow]}16
  \end{block}
&
\begin{block}{5}{20}
    \column{5}{20}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}24
    \piece{\Sq[green]}1{12}
  \end{block}
\\\\
\end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/sqrtick.tex <==
\ifredraw
\begin{tabular}{llll}
  \begin{block}{5}{12}
    \column{1}{12}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\Sq[red]}04
  \end{block} 
&
  \begin{block}{5}{12}
    \column{1}{12}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\Sq[green]}14
  \end{block} 
\\\\
\end{tabular}
\else
\includegraphics{figures/rtick/sqrtick.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/rtick/sqsqrtick.tex <==
\ifredraw
\includegraphics{figures/rtick/sqsqrtick.epsi.clean}
\begin{tabular}{llll}
  \begin{block}{5}{12}
    \column{1}{12}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\Sq[green]}14
    \piece{\Sq[red]}06
  \end{block} 
&
  \begin{block}{5}{12}
    \column{1}{12}
    \piece{\LGr[lightgray]}2{0}
    \piece{\Sq[lightgray]}1{2}
    \piece{\Sq[green]}14
    \piece{\Sq[red]}16
  \end{block} 
\\\\
\end{tabular}
\else
\includegraphics{figures/rtick/sqsqrtick.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/lg.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGu[red]}04
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGu[red]}14
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGd[yellow]}03
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGd[red]}14
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGd[red]}29
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGl[red]}04
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[red]}04
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[red]}15
\end{block}
&
\begin{block}{5}{10}
  \column{6}{10}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}25
\end{block}
\end{tabular}
\else
\includegraphics{figures/unapproachable/lg.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/lglgH.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGl[red]}04
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGl[red]}0{13}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[red]}04
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[red]}0{13}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[red]}1{17}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{17}
\end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/unapproachable/lglgH.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/lglgV.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGu[red]}04
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGu[red]}14
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGu[yellow]}1{13}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGd[yellow]}03
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGd[red]}14
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGd[yellow]}1{11}
\end{block}
&
\begin{block}{5}{22}
  \column{6}{22}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGd[red]}2{15}
\end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/unapproachable/lglgV.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/ls.tex <==
\ifredraw
\begin{tabular}{llll}
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\LSr[red]}04
\end{block}
&
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\LSr[red]}1{5}
\end{block}
&
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\LSu[yellow]}03
\end{block}
&
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\LSu[red]}14
\end{block}
\end{tabular}
\else
\includegraphics{figures/unapproachable/ls.epsi.clean}
\fi

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/lslg.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSr[red]}04
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSr[red]}1{5}
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSr[red]}0{13}
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSu[yellow]}03
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSu[red]}14
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LSu[yellow]}1{12}
\end{block}\\\\
\end{tabular}
\else
\includegraphics{figures/unapproachable/lslg.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/sq.tex <==
\ifredraw
\begin{tabular}{ll}
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\Sq[red]}04
\end{block}
&
\begin{block}{5}{8}
  \column{6}{8}
  \piece{\floor[lightgray]344}00
  \piece{\Sq[red]}14
\end{block}
\end{tabular}
\else
\includegraphics{figures/unapproachable/sq.epsi.clean}
\fi

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/sqlg.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\Sq[red]}04
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\Sq[red]}14
\end{block}
&
\begin{block}{5}{16}
  \column{6}{16}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\Sq[yellow]}1{13}
\end{block}\\\\
\end{tabular}
\else
\includegraphics{figures/unapproachable/sqlg.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/unapproachable/sqlglg.tex <==
\ifredraw
\begin{tabular}{llllllllll}
\begin{block}{5}{28}
  \column{6}{28}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{23}
  \piece{\Sq[red]}04
\end{block}
&
\begin{block}{5}{28}
  \column{6}{28}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{23}
  \piece{\Sq[red]}14
\end{block}
&
\begin{block}{5}{28}
  \column{6}{28}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{23}
  \piece{\Sq[yellow]}1{13}
\end{block}
&
\begin{block}{5}{28}
  \column{6}{28}
  \piece{\floor[lightgray]344}00
  \piece{\LGr[green]}2{11}
  \piece{\LGr[green]}2{23}
  \piece{\Sq[yellow]}1{25}
\end{block}
\\\\
\end{tabular}
\else
\includegraphics{figures/unapproachable/sqlglg.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/valid/lglgunappvalid.tex <==
\ifredraw
\begin{tabular}{llll}
% \begin{block}{5}{14}
%     \column{1}{14}
%     \piece{\floor[lightgray]455}00
%     \piece{\LGr[lightgray]}20
%     \piece{\LGr[green]}2{12}
%     \piece{\LGd[green]}1{12}
%   \end{block}
% & ~~~~~~~~~~ & 
  \begin{block}{5}{26}
    \column{1}{26}
    \piece{\floor[lightgray]455}00
    \piece{\LGr[lightgray]}20
    \piece{\LGr[green]}2{12}
    \piece{\LGr[green]}2{24}
  \end{block}
\\\\
%     ($\tLG$-UA-$i$-2) &&
($\tLG$-UA-$\{i,j\}$)\\\\
\end{tabular}
\else
\includegraphics{figures/valid/lglgunappvalid.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/lglgunpreppedvalid.tex <==
\ifredraw
\begin{tabular}{ccccccc}
\begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[green]}1{10}
  \end{block}
& & 
\begin{block}{5}{14}
    \column{5}{14}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[green]}2{10}
    \piece{\LGd[green]}1{10}
  \end{block}
& ~~~~~~~~~~ & 
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]044}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}2{22}
  \end{block}
& & 
  \begin{block}{5}{26}
    \column{5}{26}
    \piece{\floor[lightgray]440}00
    \piece{\LGr[green]}2{10}
    \piece{\LGr[green]}2{22}
  \end{block}
\\\\
     \multicolumn{2}{c}{($\tLG$-UP-$i$-2)} &&&
     \multicolumn{2}{c}{($\tLG$-UP-$\{i,j\}$)}\\\\
\end{tabular}
\else
\includegraphics{figures/valid/lglgunpreppedvalid.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/lgoverflatvalid.tex <==
    \begin{tabular}{cccccccc}
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGu[green]}06
      \end{block}
      & ~~~~~~ &
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGu[green]}16
      \end{block}
      & ~~~~~~ &
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGr[green]}06
      \end{block}
      & ~~~~~~ &
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGr[green]}2{10}
      \end{block}\\\\
      ($\tLG$-OF-1) && ($\tLG$-OF-2) && ($\tLG$-OF-3) && ($\tLG$-OF-4-$i$)\\\\
    \end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/valid/lgthappyvalid.tex <==
      \begin{tabular}{ccc}
      \begin{block}{5}{20}
        \column{5}{20}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGr[darkgreen]}06
        \piece{\LSl[darkgreen]}07
        \piece{\LGr[green]}2{16}
      \end{block}
& ~~~~~~ & 
      \begin{block}{5}{26}
        \column{5}{26}
        \piece{\floor[lightgray]044}00
        \piece{\Iu[darkgreen]}00
        \piece{\LGr[darkgreen]}24
        \piece{\Sq[darkgreen]}04
        \piece{\LGr[darkgreen]}06
        \piece{\LSl[darkgreen]}07
        \piece{\LGr[green]}2{16}
        \piece{\LGr[green]}2{22}
      \end{block}
%& ~~~~~~ & 
%      \begin{block}{5}{14}
%        \column{5}{14}
%        \piece{\floor[lightgray]044}00
%        \piece{\Iu[darkgreen]}00
%        \piece{\LGr[darkgreen]}24
%        \piece{\Sq[darkgreen]}04
%        \piece{\LGr[darkgreen]}06
%        \piece{\LSl[darkgreen]}07
%        \piece{\LGl[green]}08
%      \end{block}
\\\\
      ($\tLG$-TH-i) 
&&      ($\tLG$-TH-$\{i,j\}$)
\\\\
    \end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 


==> figures/valid/lgunappvalid.tex <==
\begin{tabular}{ccccc}
\begin{block}{5}{14}
  \column{1}{14}
  \piece{\floor[lightgray]455}00
  \piece{\LGr[lightgray]}20
  \piece{\LGr[green]}2{12}
\end{block}
\\\\
($\tLG$-UA-i)\\\\
\end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/lgunderflatvalid.tex <==
\begin{tabular}{ccccc}
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]444}00
  \piece{\LGr[green]}2{10}
\end{block}
\\\\
($\tLG$-UF-i)\\\\
\end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/lgunpreppedvalid.tex <==
\ifredraw
\begin{tabular}{lllllll}
      \begin{block}{5}{8}
        \column{5}{8}
        \piece{\floor[lightgray]044}00
        \piece{\Ir[green]}14
      \end{block}
&
      \begin{block}{5}{14}
        \column{5}{14}
        \piece{\floor[lightgray]440}00
        \piece{\Ir[green]}1{10}
      \end{block}
& ~~~~~~ &
      \begin{block}{5}{8}
        \column{5}{8}
        \piece{\floor[lightgray]440}00
        \piece{\Iu[green]}04
      \end{block}
& ~~~~~~~~~ &
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]044}00
  \piece{\LGr[green]}2{10}
\end{block}
&
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]440}00
  \piece{\LGr[green]}2{10}
\end{block}
\\\\
($\tI$-UP-1-$i$) &&& ($\tI$-UP-2) && ($\tLG$-UP-i)
\\\\
\end{tabular}
\else
\includegraphics{figures/valid/lgunpreppedvalid.epsi.clean}
\fi


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/lgunvalid.tex <==
\begin{tabular}{ccccc}
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]044}00
  \piece{\LGr[green]}2{10}
\end{block}
& ~~~~~~ & 
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]440}00
  \piece{\LGr[green]}2{10}
\end{block}
& ~~~~~~ & 
\begin{block}{5}{14}
  \column{5}{14}
  \piece{\floor[lightgray]044}00
  \piece{\LGr[green]}2{10}
  \piece{\Iu[darkgreen]}00
\end{block}
\\\\
($\tLG$-UP-i) &&  ($\tLG$-UP-i) && ($\tLG$-UF-i)\\\\
\end{tabular}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tetris"
%%% End: 



==> figures/valid/valid1.tex <==
\ifredraw
\psset{unit=0.04in}
\setlength{\tabcolsep}{-2pt}
\[
\underbrace{
  \begin{tabular}{ccccccccccccccccccccccc}
    \begin{block}{4}{30}
      \column{5}{30}
    \piece{\floor[lightgray]440}00
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]440}00
    \piece{\Iu[green]}20
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]444}00
    \piece{\LGr[green]}24
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]444}00
    \piece{\LGr[lightgray]}24
    \piece{\Sq[green]}04
  \end{block}
\end{tabular}
}_{\mbox{initiator}}
\]

\begin{tabular}{ccccccccccccccccccccccc}
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]666}00
    \piece{\LGr[lightgray]}24
    \piece{\LGr[green]}06
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]877}00
    \piece{\LGr[lightgray]}24
    \piece{\LSl[green]}07
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]998}00
    \piece{\LGr[lightgray]}24
    \piece{\LGl[green]}08
  \end{block}
%\\\\
%\end{tabular}%
\else
\includegraphics{figures/valid/valid1.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 


==> figures/valid/valid2.tex <==
\ifredraw%
%\begin{tabular}{ccccccccccc}
&
\begin{block}{4}{30}
    \column{5}{30}
    \piece{\floor[lightgray]{10}{10}{10}}00
    \piece{\LGr[lightgray]}24
    \piece{\LGr[green]}2{10}
  \end{block}
   &
   \begin{block}{4}{30}
     \column{5}{30}
     \piece{\floor[lightgray]{10}{10}{10}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\Sq[green]}0{10}
   \end{block}
   &
   \begin{block}{4}{30}
     \column{5}{30}
     \piece{\floor[lightgray]{12}{12}{10}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\LGr[green]}0{12}
   \end{block}\\\\
% \end{tabular}%
%\begin{tabular}{ccccccccccc}
  \begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{14}{13}{13}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\LSl[green]}0{13}
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{15}{15}{14}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
    \piece{\LGl[green]}0{14}
  \end{block}
  &
  \begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
    \piece{\annotation{\vdots}}{1.5}{17}
  \end{block}
%\\\\
%\end{tabular}
\else
\includegraphics{figures/valid/valid2.epsi.clean}
\includegraphics{figures/valid/valid2.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 


==> figures/valid/valid3.tex <==
\ifredraw
%\begin{tabular}{ccccccccccc}
&
  \begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
  \end{block}
&
\begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
     \piece{\LGr[green]}2{22}
  \end{block}
&
\begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
     \piece{\LGr[lightgray]}2{22}
     \piece{\Sq[green]}0{22}
  \end{block}
&
\begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
     \piece{\floor[lightgray]222}0{22}
     \piece{\LGr[lightgray]}2{22}
     \piece{\Sq[green]}0{24}
  \end{block}
&
\begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
     \piece{\floor[lightgray]442}0{22}
     \piece{\LGr[lightgray]}2{22}
     \piece{\Sq[green]}0{26}
  \end{block}
&
\begin{block}{4}{30}
    \column{5}{30}
     \piece{\floor[lightgray]{16}{16}{16}}00
     \piece{\LGr[lightgray]}24
     \piece{\LGr[lightgray]}2{10}
     \piece{\annotation{\vdots}}{1.5}{17}
     \piece{\LGl[lightgray]}0{20}
     \piece{\floor[lightgray]662}0{22}
     \piece{\LGr[lightgray]}2{22}
  \end{block}\\\\
\end{tabular}
\else
\includegraphics{figures/valid/valid3.epsi.clean}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../../tetris"
%%% End: 

